Consistent regression when oblivious outliers overwhelm

We consider a robust linear regression model $y=X\beta^* + \eta$, where an adversary oblivious to the design $X\in \mathbb{R}^{n\times d}$ may choose $\eta$ to corrupt all but an $\alpha$ fraction of the observations $y$ in an arbitrary way. Prior to our work, even for Gaussian $X$, no estimator for $\beta^*$ was known to be consistent in this model except for quadratic sample size $n \gtrsim (d/\alpha)^2$ or for logarithmic inlier fraction $\alpha\ge 1/\log n$. We show that consistent estimation is possible with nearly linear sample size and inverse-polynomial inlier fraction. Concretely, we show that the Huber loss estimator is consistent for every sample size $n= \omega(d/\alpha^2)$ and achieves an error rate of $O(d/\alpha^2n)^{1/2}$. Both bounds are optimal (up to constant factors). Our results extend to designs far beyond the Gaussian case and only require the column span of $X$ to not contain approximately sparse vectors). (similar to the kind of assumption commonly made about the kernel space for compressed sensing). We provide two technically similar proofs. One proof is phrased in terms of strong convexity, extending work of [Tsakonas et al.'14], and particularly short. The other proof highlights a connection between the Huber loss estimator and high-dimensional median computations. In the special case of Gaussian designs, this connection leads us to a strikingly simple algorithm based on computing coordinate-wise medians that achieves optimal guarantees in nearly-linear time, and that can exploit sparsity of $\beta^*$. The model studied here also captures heavy-tailed noise distributions that may not even have a first moment.

==> content/tsakonas.tex <==
\section{Generalization of the proof from \cite{tsakonas2014convergence}}\label{sec:results}
\subsection{Sketch of their proof}
The model is 
\[
\pmb y = \pmb X\betastar + \pmb w +  \zeta \,,
\]
where
$\pmb X \sim N(0,1)^{n\times d}$, $\pmb w\in N(0,1)^n$ is independent of $\pmb X$, $\betastar \in \R^d$, $\zeta\in \R^n$ is a deterministic $(1-\alpha)n$-sparse vector for some $\alpha \in (0,1)$. 
As usual, $\pmb X$ and $\pmb y$ are known, and the goal is to recover $\betastar$. We assume that $d = o(\alpha^2 n)$ (otherwise there is no consistent estimator).

\cite{tsakonas2014convergence}  study the Huber loss function
\[
\pmb L(\beta) = \sum_{i=1}^n \Phi\Paren{\pmb y_i - \iprod{\pmb X_i,\beta}} = 
\sum_{i=1}^n \Phi\Paren{\iprod {\pmb X_i, {\betastar - \beta}} + \pmb w_i +  \zeta_i}\,,
\]
where $\Phi(t) = t^2/2$ for $\abs{t}\le 1$ and $\Phi(t) = \abs{t} - 1/2$ for $\abs{t}> 1$.

They consider the ball $\cB$ centered at $\betastar$ of radius 
$r = \frac{C}{\alpha} \sqrt{\frac{d}{n}}$ for some large enough absolute constant $C$. 
They define the set 
\[
\pmb\cA = \Set{i\in [n]\suchthat \zeta_i=0,\, \abs{\pmb w_i} \le 0.5,\, 
	\norm{\pmb X_i}\le \frac{1}{2r}}\,.
\]
For any $i\in \pmb\cA$ the corresponding term of the Huber function is quadratic for all $\beta \in \cB$. Indeed, by C--S inequality, for all $\beta \in \cB$, 
$\Abs{\iprod {\pmb X_i, {\betastar - \beta}} + \pmb w_i +  \zeta_i} \le 1$.

Since whp for all $i\in [n]$,  $\norm{\pmb X_i} = \sqrt{d} \pm O\Paren{\sqrt{\log n}}$, the set 
$\pmb\cA$ is empty if $\sqrt{d} \gtrsim  \alpha \sqrt{\frac{n}{d}}$, 
i.e. when $n \lesssim \frac{d^2}{\alpha^2}$ (here we assume for simplicity that $\alpha \ge \sqrt{\frac{\ln n}{n}}$). 
Moreover, if $n \lesssim \frac{d}{\alpha^2}$, then the set of $i\in [n]$ 
such that the corresponding term in the Huber function is quadratic for all $\beta \in \cB$ is also empty: for each $i\in[n]$ we can take $\beta$ such that $\betastar-\beta$ is parallel to $\pmb X_i$.

Further we assume $n \gtrsim \frac{d^2\ln n}{\alpha^2}$. 
Note that the condition $\norm{\pmb X_i}\le \frac{1}{2r}$ whp holds for all $i\in [n]$, 
hence $\pmb \cA$ is independent of $\pmb X$.
It follows that whp $\Card{\pmb\cA}\ge \Omega\Paren{\alpha n}$, 
so the minimal eigenvalue of $\transpose{\pmb X_{\pmb \cA}}\pmb X_{\pmb \cA}$  satisfies
$\lambda_{\min}\Paren{\transpose{\pmb X_{\pmb \cA}}\pmb X_{\pmb \cA}} \ge \Omega(\alpha n)$ (here we use $d=o(\alpha n)$).

For $\beta\in \R^d$ denote 
$\pmb L_1(\beta) =  \sum_{i\in \pmb \cA} \Phi\Paren{\pmb y_i - \iprod{\pmb X_i,\beta}}$ and 
$\pmb L_2(\beta) =  \sum_{i\notin \pmb \cA} \Phi\Paren{\pmb y_i - \iprod{\pmb X_i,\beta}}$. 
By convexity, 
\[
\pmb L_2(\beta) \ge \pmb L_2(\betastar) + \iprod{\nabla \pmb L_2(\betastar), {\beta-\betastar}}\,.
\]
Since $\pmb L_1(\beta)$ is quadratic, 
\[
\pmb L_1(\beta) \ge \pmb L_1(\betastar) + \iprod{\nabla \pmb L_1(\betastar), {\beta-\betastar}} + 
\frac{1}{2}\lambda_{\min}
\Paren{\transpose{\pmb X_{\pmb \cA}}\pmb X_{\pmb \cA}}\Snorm{\beta - \betastar}\,.
\]
Hence
\[
\pmb{L}(\beta) \ge \pmb L(\betastar) + \iprod{\nabla \pmb L(\betastar), {\beta-\betastar}} + 
\Omega(\alpha n)\cdot\Snorm{\beta - \betastar}\,.
\]

Let $\pmb \beta'$ be a minimizer of $\pmb L$ in $\cB$. Then
\[
 \iprod{\nabla \pmb L(\betastar), {\beta'-\betastar}} + 
\Omega(\alpha n)\cdot\Snorm{\beta' - \betastar} \le 0\,.
\]
It follows that
\[
\norm{\beta' - \betastar} \le O\Paren{\frac{1}{\alpha n}\norm{\nabla \pmb L(\betastar)}}\,.
\]

Since $\pmb X \sim N(0,1)^{n\times d}$, 
the distribution of $\nabla \pmb L(\betastar)$ given $\pmb w$ is 
$N\Paren{0,\sum_{i=1}^n \phi^2\Paren{\zeta_i + \pmb w_i} \cdot \Id_d}$, where $\phi(t) = \Phi'(t)$. Hence with probability at least $0.99$,
$\norm{\nabla \pmb L(\betastar)} \le O(\sqrt{nd})$. If $C$ is large enough, we get 
$\norm{\beta' - \betastar} \le r/2$, hence $\beta'$ is in the interior of $\cB$ and by convexity is also a global minimum of $\pmb L(\beta)$. So with probability at least $0.99$ the Huber loss minimizer $\betahat$ satisfies
\[
\norm{\betahat-\betastar} \le \frac{C}{\alpha} \sqrt{\frac{d}{n}}
\]
for some large enough absolute constant $C$.

\subsection{The case $n<d^2/\alpha^2$.}
Consider the global Huber minimizer $\pmb \betahat$ and let $\pmb \beta'$ be a minimum of $\pmb L$ over the interval $\cI = \cB\cap\Set{\beta\in \R^d\suchthat 
	\exists t\ge 0\quad \beta - \betastar = t\Paren{\pmb \betahat - \betastar}}$. 
Define the set 
\[
\pmb \cC = \Set{i\in [n]\suchthat \zeta_i=0,\, \abs{\pmb w_i} \le 0.5}\,.
\]
and the set
\[
\pmb \cS = \pmb\cC\cap
\Set{i\in [n]\suchthat\Abs{\iprod{\pmb X_i, {\betastar - \pmb \beta'}}} \le 0.5}\,.
\]

$\pmb \cC$ is independent of $\pmb X$ and whp has size $\Omega(\alpha n)$, hence whp 
$\lambda_{\min}\Paren{\transpose{\pmb X_{\pmb \cC}}\pmb X_{\pmb \cC}}
\ge \Omega\Paren{\alpha n}$. 
Since the $k$-sparse norm of a Gaussian matrix $\transpose{\pmb X_{\pmb \cC}}$ is at most $\sqrt{d} + 10\sqrt{k\ln(e\cdot\card{\pmb \cC}/k)}$, the average absolute value among top 
$0.001\cdot\card{\pmb \cC}$ coordinates of 
$\pmb X_{\pmb \cC}\Paren{\betastar - \pmb\beta'}$ is at most $100 r \le 0.5$, 
hence $\card{\pmb\cS} \ge 0.999 \cdot\card{\pmb \cC} \ge \Omega\Paren{\alpha n}$. 
Moreover, since $d=o(\alpha n)$, whp
$
\lambda_{\min}\Paren{\transpose{\pmb X_{\pmb \cS}}\pmb X_{\pmb \cS}}
\ge \Omega\Paren{\alpha n}
$.

Then the same argument as in the original proof shows that with probability at least $0.99$, $\pmb \beta'$ is an inner point of the interval $\cI$, and there is a point $\beta'' \in \cI$ such that $\pmb L(\beta'') > \pmb L (\pmb \beta')$. By convexity, $\pmb \betahat \in \cI$ and we get the desired bound.


\subsection{Non-Gaussian design}
We assume that $X$ is deterministic and satisfies RIP: 
for any set $\cR\subset [n]$ of size at most $C\cdot\frac{d\ln  n}{\alpha^2}$ and for any $u\in \R^d$,
\[
\norm{X_R u} \le \frac{1}{C}\cdot \norm{Xu}\,,
\]
for large enough constant $C>0$.

For deterministic $X$ we need some assumptions on the noise. We assume that $\pmb \zeta$ is obtained from some (arbitrary) $(1-\alpha)n$-sparse vector by applying random permutation and randomly flipping signs of entries of this vector (sampling permuation, flipping signs and $\pmb w$ are all mutually independent).

Also, wlog we can assume $\transpose{X}X = n\Id$. Obeserve that for any unit $u\in \R^d$, $||X_{\pmb \cC}u||\le 10\cdot\sqrt{\alpha n}$. Indeed, for fixed $u$ we have this bound with probability $1- 2^{-\Omega(\alpha n)}$, and it is enough to consider a $0.5$-net on the unit sphere in $\R^d$, which has size $2^{O(d)}$ (recall that we assume $\alpha n \gg d$). Moreover, since RIP can be defined only in terms of $u$ (we can take top coordinates of $Xu$ as $\cR$), we get that for any unit $u\in \R^d$,
\[
||X_{\pmb\cC\cap R} u || \le \frac{10}{C} \cdot \sqrt{\alpha n}
\]
whp.

Let $\pmb \beta'$ and $\pmb\cS$ be as in the previous section 
and denote $\pmb u = \pmb\beta' - \betastar$.
We have
\[
\pmb L(\pmb \beta') \ge \pmb L(\betastar) +  \iprod{\nabla \pmb L(\betastar), {\pmb u}} + 
\frac{1}{2}\Snorm{ X_{\pmb \cS}\pmb u}
=  \pmb L(\betastar) + \iprod{\pmb v,  X\pmb u} + 
\frac{1}{2}\Snorm{X_{\pmb \cS}\pmb u}
\,,
\]
where $\pmb v$ is a vector with coordinates $\pmb v_i = \phi(\pmb\zeta_i + \pmb w_i)$. By Hoeffding's inequality (with a union bound over $u\in \cB$), whp
\[
\abs{\iprod{\pmb v,  X\pmb u}}\le O\Paren{\norm{X\pmb u} \sqrt{d\log n} + 1}\,.
\]
Hence
\[
\Snorm{X_{\pmb \cS}\pmb u} \le O\Paren{\norm{X\pmb u} \sqrt{d\log n} + 1}\,.
\]

Now consider the set $\pmb\cT$ of the top $d/\alpha^2$ coordinates (by abs value) of $X\pmb u$. Then 
\[\norm{X_{\pmb \cC \cap \pmb \cT} \pmb u} \le 10\cdot\frac{1}{C}\sqrt{\alpha n}\cdot \norm{u}\le \frac{10}{C} \sqrt{\alpha n}\cdot r \le \sqrt{d/\alpha}\,.\] 
The size of $\pmb \cC \cap \pmb \cT$ is at most $d/\alpha$, hence the average squared coordinate in $\pmb \cC \cap \pmb \cT$ is at most $1$. So $\pmb \cS$ contains  $\pmb \cC\setminus \pmb \cT$, and $\Snorm{X_{\pmb \cS}\pmb u}\ge 0.1 \alpha \cdot \Snorm{X\pmb u}$ (for large enoug $C$). 
Putting everything together, we get
\[
\norm{X\pmb u} \le O\Paren{\frac{\sqrt{d\log n}}{\alpha}}\,.
\]

%Assume that $\Snorm{X_{\pmb \cS}\pmb u} < 0.1 \cdot\alpha\cdot\Snorm{X\pmb u}$. 

